Languages You Know Influence Those You Learn: Impact of Language Characteristics on Multi-Lingual Text-to-Text Transfer

Multi-lingual language models (LM), such as mBERT, XLM-R, mT5, mBART, have been remarkably successful in enabling natural language tasks in low-resource languages through cross-lingual transfer from high-resource ones. In this work, we try to better understand how such models, specifically mT5, transfer *any* linguistic and semantic knowledge across languages, even though no explicit cross-lingual signals are provided during pre-training. Rather, only unannotated texts from each language are presented to the model separately and independently of one another, and the model appears to implicitly learn cross-lingual connections. This raises several questions that motivate our study, such as: Are the cross-lingual connections between every language pair equally strong? What properties of source and target language impact the strength of cross-lingual transfer? Can we quantify the impact of those properties on the cross-lingual transfer? In our investigation, we analyze a pre-trained mT5 to discover the attributes of cross-lingual connections learned by the model. Through a statistical interpretation framework over 90 language pairs across three tasks, we show that transfer performance can be modeled by a few linguistic and data-derived features. These observations enable us to interpret cross-lingual understanding of the mT5 model. Through these observations, one can favorably choose the best source language for a task, and can anticipate its training data demands. A key finding of this work is that similarity of syntax, morphology and phonology are good predictors of cross-lingual transfer, significantly more than just the lexical similarity of languages. For a given language, we are able to predict zero-shot performance, that increases on a logarithmic scale with the number of few-shot target language data points.

==> figures/data_lang_last.tex <==
\begin{table}[h]
	\footnotesize
	\centering
	\scalebox{1.0}{ 
		\begin{tabular}{lrrr}
			\toprule
			&  \multicolumn{3}{c}{\underline{Available Data Train/Test}} \\
			Languages (iso)&XNLI &  TyDiQA & NER \\ 
			\midrule
			Arabic (AR) & 1/1 & 1/1 &   1/1  \\
			Bengali (BN) & $\emptyset$  & 1/1 &  $\emptyset$  \\
			English (EN) & 1/1  & 1/1 & 1/1  \\
			Finnish (FI) & $\emptyset$  & 1/1 &   1/1 \\
			Indonesian (ID) & $\emptyset$  & 1/1 & 1/1  \\
			%KO & $\emptyset$  & 1/1 & 1/1 \\
			Russian (RU) & 1/1  & 1/1 & 1/1  \\
			Swahili (SW) & 1/1  & 1/1  &$\emptyset$/1   \\
			%\hdashline
			%\multicolumn{6}{c}{\textit{Extension: complementing to have full task coverage for each language family}}\\
			Spanish (ES) & 1/1  & $\emptyset$  & 1/1   \\
			German (DE) & 1/1  & $\emptyset$   & 1/1  \\
			Hindi (HI) & 1/1  & $\emptyset$   & 1/1  \\
			%YO & $\emptyset$  & $\emptyset$ & $\emptyset$  & $\emptyset$  & 1/1 \\
			%\hdashline
			%\multicolumn{1}{c}{\textit{Extension}}\\
			%TR & 1/1  & $\emptyset$ & $\emptyset$  & 1/1  & 1/1 \\
			%ZH & 1/1  & $\emptyset$ & 1/1  & 1/1  & 1/1 \\
			\bottomrule
		\end{tabular}
	}
	\caption{Annotated Data available per studied tasks for languages included in mT5 pretraining. The selection was done starting on the TyDiQA languages and extended to have a better coverage across all tasks. 1/1 means that data is available for both training and evaluation. $\emptyset$/1 means it is only available for evaluation. 
	%NB: Hindi could be added to palliate the lack of annotated data for Bengali in XNLI and NER (Indo-Aryan language family). \\
	%NB: Yoruba could be added to palliate the lack of annotated data for Swahili in XNLI and NER (Niger-Congo language family). \\
	%*for MLQA training data is the SQUAD-1.1 dataset for English and the MLQA dev set for few shot learning for other languages. For this reason, MLQA should only be used for complementing TyDiQA
	}
	\label{tab:data_langs}
\end{table}
